FedNLP: Benchmarking Federated Learning Methods for Natural Language Processing Tasks

Increasing concerns and regulations about data privacy and sparsity necessitate the study of privacy-preserving, decentralized learning methods for natural language processing (NLP) tasks. Federated learning (FL) provides promising approaches for a large number of clients (e.g., personal devices or organizations) to collaboratively learn a shared global model to benefit all clients while allowing users to keep their data locally. Despite interest in studying FL methods for NLP tasks, a systematic comparison and analysis is lacking in the literature. Herein, we present the FedNLP, a benchmarking framework for evaluating federated learning methods on four different task formulations: text classification, sequence tagging, question answering, and seq2seq. We propose a universal interface between Transformer-based language models (e.g., BERT, BART) and FL methods (e.g., FedAvg, FedOPT, etc.) under various non-IID partitioning strategies. Our extensive experiments with FedNLP provide empirical comparisons between FL methods and helps us better understand the inherent challenges of this direction. The comprehensive analysis points to intriguing and exciting future research aimed at developing FL methods for NLP tasks.

==> tex/_alg_fl.tex <==
\begin{algorithm}[t]
    % \setstretch{1.35}
% 	\small
	\nonl \textbf{Notation:}  {$N=$ \# clients, $R=$ \# rounds of communication, $E=$ \# epochs; $B=$ sample size;  $\mathcal{D}_i$ and $\mathcal{M}_i$ as the local dataset and model of client $C_i$; $M_i^t$ are models at $t$-th round; learning rate $\eta$.} 
% 	\comm{is a probe that has $|\mathcal L|$ sub-sets; each sub-set $M^{l_x}$ is a set of $K$ assertions in the same language $l_x\in \mathcal{L}$. $M^{l_x}_t$ is always the truth.}
    ~\\
	\nonl \textbf{In}: {$\{\mathcal{D}_1, \mathcal{D}_2, \dots, \mathcal{D}_N\}$}. 
	~\\
	\nonl \textbf{Out}: $M_G^R$, the global model shared by all clients after $R$ rounds of aggregation.
	%	\nonl {\scriptsize{/*~~*/}}
	
	$M_G^0.\operatorname{initialize()}$ \comm{Initialize a global model.} \\ 
	\For{$t = 0, 1, ..., R-1$ } { 
	    \comm{Sample $B$ clients from the total clients.} \\
	    $\mathcal{S}_t \leftarrow \Gamma(N, B)$ \\
	    \comm{Get \# examples in sampled clients.} 
	    $n \xleftarrow[]{} \sum_{i\in \mathcal{S}_t} |\mathcal{D}_i|$ \\ 
	    \ForEach{$c \in \mathcal{S}_t$ \underline{\textbf{in parallel}}}{ 
	        $M_i^t \leftarrow M_G^t$~~\comm{Sync the local model.} \\ 
	        $M_i^t.\operatorname{train(\mathcal{D}_i, E, \eta)}$ \comm{Locally train.} \\ 
	        $\Delta_i \leftarrow M_i^t - M_G^t$ \\
	       % \hspace{50em}\raisebox{.5\baselineskip}[0pt][0pt]{$\left.\rule{0pt}{3.2\baselineskip}\right\}\ \mbox{in parallel}$}
	       \comm{Send the local updates $\Delta_i$ to server.}
	    }
	    $M_G^{t+1} \leftarrow M_G^{t} + \eta \sum_{i \in \mathcal{S}_t} \frac{\left|\mathcal{D}^{i}\right|}{n} \Delta_i $ \\
	    \comm{Until all clients in $\mathcal{S}_t$ finished local training, update the current global model by averaging the updates of all local client models.}
	}
% 	 $l_a \xleftarrow{}\Gamma_{1}(\mathcal{L})$ ~\comm{Pick an anchor language.} \\
% 	 $C \xleftarrow{} \{M^{l_a}_t\}$ \comm{Initiate w/ the truth assertion.} \\
% 	\comm{Iterate each sampled distractor language $l_i$.} \\ 
% 	\ForEach{$l_i \in \Gamma_{V-1}(\mathcal{L}-{l_a})$ } { 
% 	 \comm{Sample an index of distractor assertion.}\\
% 		$j\xleftarrow{}\Gamma_{1}(\mathbb{N}_{\leq K} - \{t\})$ \\
% 		\comm{Add a distractor assertion as a candidate.}\\
% 		${C}$\text{.add}($M^{l_i}_j$)
% 	}
	\caption{{\textsc{FedAvg} algorithm for FL.}}\label{alg:fedavg}
\end{algorithm}

==> tex/_fig_jsdbetweenclients.tex <==
\begin{figure}[t]
\centering
% \hspace{-1.5em}
{\includegraphics[width=0.9\linewidth]{figure/labelshift_density.pdf}}
\caption{The probability density of the JS-divergence between 100 clients (reduced by summing on each client) on the \textit{20News} dataset with different $\alpha$ --- i.e., the matrices in Figure~\ref{fig:jsdbetweenclients}. }
\label{fig:jsdbetweenclients}
\end{figure}


==> tex/_tab_sideresults.tex <==
\begin{table}[t]
\label{tab:results}
\centering
\scalebox{0.67
	}{
\begin{tabular}{c|c||ccc|c}
\toprule
\textbf{Model} & \textbf{PT-Weights} & \textbf{FedAvg} & \textbf{FedOpt} & \textbf{FedNova} & \textbf{Central}. \\ \midrule
DistilBERT & frozen &  &  &  &  \\
BERT-base & frozen &  &  &  &  \\ \midrule
DistilBERT & trainable &  &  &  &  \\
BERT-base & trainable &  &  &  & \\ \bottomrule 
\end{tabular}
}
\caption{Experimental results for investigating performance under different models with frozen/trainable pre-trained weights.}
\end{table}

% shorturl.at/foM08
